Variance Reduced Training with Stratified Sampling for Forecasting Models

In large-scale time series forecasting, one often encounters the situation where the temporal patterns of time series, while drifting over time, differ from one another in the same dataset. In this paper, we provably show under such heterogeneity, training a forecasting model with commonly used stochastic optimizers (e.g. SGD) potentially suffers large variance on gradient estimation, and thus incurs long-time training. We show that this issue can be efficiently alleviated via stratification, which allows the optimizer to sample from pre-grouped time series strata. For better trading-off gradient variance and computation complexity, we further propose SCott (Stochastic Stratified Control Variate Gradient Descent), a variance reduced SGD-style optimizer that utilizes stratified sampling via control variate. In theory, we provide the convergence guarantee of SCott on smooth non-convex objectives. Empirically, we evaluate SCott and other baseline optimizers on both synthetic and real-world time series forecasting problems, and demonstrate SCott converges faster with respect to both iterations and wall clock time.

==> section/convergence_analysis.tex <==
\section{Convergence Analysis}
We make the following assumptions here:
\begin{enumerate}
	\item \textbf{Lipschitzian Gradient}: All the function $f_i$ have $L_i$-Lipschitzian gradients.\label{Assumption1}
	\begin{displaymath}
	\left\|\nabla f_i(x) - \nabla f_i(y)\right\|\leq L_i\left\|x-y\right\|, \forall i\in [n]
	\end{displaymath}
	And define $L=\max_i\{L_i\}$.
	\item \textbf{Spectral Gap}: Communication matrix $W$ is a symmetric doubly stochastic matrix and for $\rho\triangleq\max\{|\lambda_2(W)|, |\lambda_n(W)|\}$, $\rho<1$.\label{Assumption2}
	\item \textbf{Bounded Variance}:
		%\begin{displaymath}
			\begin{align*}
			& \mathbb{E}_{\xi_i\sim\mathcal{D}_i}\left\|\nabla\widetilde{f}_i(x;\xi_i) - \nabla f_i(x)\right\|^2 \leq \sigma^2, \forall i\\
			& \mathbb{E}_{i\sim\mathcal{U}([n])}\left\|\nabla f_i(x) - \nabla f(x)\right\|^2 \leq \varsigma^2, \forall i\\
			\end{align*}
		%\end{displaymath}
		For one worker, the first inequality shows that inter variance is bounded by some constant $\sigma^2$. The second inequality shows intra variance is bounded by some constant $\varsigma^2$. \label{Assumption3}
	\item \textbf{Initialization}: All the workers start from the same point, and without the loss of generality, we have $x_{0,i}=0, \forall i$ \label{Assumption4}
	\item \textbf{Bounded sample gradient norm}: For any subgradient $\widetilde{g}_{k,i}$ sampled by $i$ at iteration $k$, we have$\left\|\widetilde{g}_{k,i}\right\|\leq G, \forall i$ \label{Assumption4}
\end{enumerate}
\begin{theorem}\label{QD-PSGD rate}
If we apply a general quantizer $\mathcal{Q}$ (can be biased, non-linear) such that $\left\|\mathcal{Q}(z)-z\right\|^2\leq\omega^2\left\|z\right\|^2, \forall z\in\mathbb{R}^d$, where $\omega$ is a hyper parameter associated with the quantizer, make the exchanged information
\begin{displaymath}
q_{k,i}=\theta\mathcal{Q}\left(\frac{x_{k,i}}{\theta}\mod 1\right)
\end{displaymath}
And by setting $\theta=\frac{16\log(4n)\alpha G}{1-\rho}$, $\omega=\frac{1-\rho}{32\log(4n)}$ and $\alpha=\frac{1}{\varsigma^{\frac{2}{3}}K^{\frac{1}{3}}+\sigma\sqrt{\frac{K}{n}}}$, the output of Quantized D-PSGD has
\begin{equation}
%\begin{align*}
	\frac{1}{K}\sum_{k=0}^{K-1}\mathbb{E}\left\|\nabla f(\overline{X}_k)\right\|^2\lesssim \frac{\sigma}{\sqrt{nK}} + \frac{\varsigma^{\frac{2}{3}}}{K^{\frac{2}{3}}} + \frac{n}{K} + \frac{nG^2}{\sigma^2K}
%\end{align*}
\end{equation}
\end{theorem}
\paragraph{Remark 1} Note that comparing the asymptotic rate in Theorem~\ref{QD-PSGD rate} with D-PSGD \cite{lian2017can}, the quantization noise introduces $\frac{nG^2}{\sigma^2K}$, which is dominated by $\frac{\sigma}{\sqrt{nK}}$ when $K$ is sufficient large. And 
\begin{corollary}
If we use a linear quantizer with quantization length $\delta$, the number of bits required per dimension per iteration is
\begin{displaymath}
    \log\left(\frac{32\log(4n)\sqrt{d}}{1-\rho}\right)
\end{displaymath}
\end{corollary}
